Planning for Attacker Entrapment in Adversarial Settings

In this paper, we propose a planning framework to generate a defense strategy against an attacker who is working in an environment where a defender can operate without the attacker's knowledge. The objective of the defender is to covertly guide the attacker to a trap state from which the attacker cannot achieve their goal. Further, the defender is constrained to achieve its goal within K number of steps, where K is calculated as a pessimistic lower bound within which the attacker is unlikely to suspect a threat in the environment. Such a defense strategy is highly useful in real world systems like honeypots or honeynets, where an unsuspecting attacker interacts with a simulated production system while assuming it is the actual production system. Typically, the interaction between an attacker and a defender is captured using game theoretic frameworks. Our problem formulation allows us to capture it as a much simpler infinite horizon discounted MDP, in which the optimal policy for the MDP gives the defender's strategy against the actions of the attacker. Through empirical evaluation, we show the merits of our problem formulation.

==> furtherMaterials/AAMAS_Stuff/1-introduction.tex <==
\section{Introduction}




In the cybersecurity community, honeypots are known to play a crucial role in developing defense strategies against attackers. As the name suggests, honeypots are used to lure and trap black hat attackers by simulating a real production system that the attackers can penetrate in and interact with. Honeypots can be either used as a defense mechanism to divert the attacker from a real system and trap them or they can be used to study an attacker's strategies in order to develop stronger security mechanisms. We are interested in the former type of honeypot. In this paper, we model the game of trapping an attacker in a honeypot as an MDP (Markov Decision Process) and show how optimal planning can help a defender capture a black hat intruder and foil their attack on the system.

<Talk about why this is useful in context of existing works>

In our planning framework, we consider two agents: an attacker and a defender. Given a honeypot-like environment, the attacker is unaware of the presence of a defender in the system and does not suspect that they are being tracked. Meanwhile, the objective of the defender is to maintain the attacker's false belief while guiding the attacker toward a trap. The system has several trap states from which the attacker cannot cause any harm. The defender's objective is achieved when the attacker is caught in one of these states. 
